Coverage Semantics for Dependent Pattern Matching

Dependent pattern matching is a key feature in dependently typed programming. However, there is a theory-practice disconnect: while many proof assistants implement pattern matching as primitive, theoretical presentations give semantics to pattern matching by elaborating to eliminators. Though theoretically convenient, eliminators can be awkward and verbose, particularly for complex combinations of patterns. This work aims to bridge the theory-practice gap by presenting a direct categorical semantics for pattern matching, which does not elaborate to eliminators. This is achieved using sheaf theory to describe when sets of arrows (terms) can be amalgamated into a single arrow. We present a language with top-level dependent pattern matching, without specifying which sets of patterns are considered covering for a match. Then, we give a sufficient criterion for which pattern-sets admit a sound model: patterns should be in the canonical coverage for the category of contexts. Finally, we use sheaf-theoretic saturation conditions to devise some allowable sets of patterns. We are able to express and exceed the status quo, giving semantics for datatype constructors, nested patterns, absurd patterns, propositional equality, and dot patterns.

==> extensions.tex <==
% !TEX root =  main.tex


\section{Extension: Support for With Clauses}

Here, we show the first steps towards supporting with-patterns~\citep{mcbrideViewLeft2004}
using coverage semantics.
Agda-style with-patterns case split on an expression's value,
looking for occurrences of it within the context and goal, then replacing them
with the matched patterns in each branch.
As such, they cannot be described using coverages alone, which
only talk about the left-hand side of a pattern match, not the right.
However, in an extensional model, the propositional equalities we construct
below can be turned into meta-equalities, and hence show
that the rewritten goal type has the same denotation
as the original one.

\subsection{Intermediate Expression Matching and Base Change}

Just like with pattern matching on equality, the key property we need
for with expressions is base change.
Consider a scrutinee context $\G$ containing the variables
whose values we are matching on, and an arrow
$g : \G -> \D $.
In the case that $\D$ is a sequence of context extensions, we can view $g$ as a dependent pair
containing values for each type in $\D$ that may refer to variables
from $\G$. So we can use the arrow $g$ to represent the intermediate expressions on which we match
 in the with-clause.

Consider now canonical cover $\{f_{i} : \D_{i} -> \D\}$, denoting the patterns
we want to match the intermediate expression(s) against.
If we are working in a category $\McC$ that has all pullbacks,
then the base change property of coverages lets us transform this cover of $\D$
into one on $\G$ by pulling back along $g$.
That is, $\{ g^{*}f_{i} : g^{*}\D_{i} : \G\}$ is a canonical cover of $\G$.

As we saw in \cref{subsec:eq-pullback}, the pullback $g^{*}f_{i}$ is
can be viewed as the most general unifier of $g$ and $f_{i}$,
giving values for the variables in both $\G$ and $\D_{i}$ that equate $f_{i}$ and $g$,
where $g^{*} \D_{i}$ contains variables from $\D_{i}$ and $\G$ that are not constrained by the unification.

In terms of with-clauses, for $T \in \Ty{\G}$ we can imagine something like this
\begin{flalign*}
  & someFunction : (\seq{x} : \G ) -> T(x) \\
  & someFunction\ \seq{x}\ \mathsf{ with }\ \applySub{g}{\seq{x}}\\
  & .(g^{*}f_{1}) \mid f_{1} = \ldots\\
  & \vdots \\
  & .(g^{*}f_{n}) \mid f_{n} = \ldots
\end{flalign*}
To define a function with $\G$ arguments, we can use an intermediate function $g$
that refers to those arguments in $\G$.
Instead of pattern matching on the function arguments, we can match the result of $g$
against covering patterns $\{f_{i}\}$,
using unification (pullback) to obtain the values that each argument must have
(i.e. dot patterns).
So long as we can compute this unification, we only need a branch for each $f_{i}$.
The base change property guarantees that this cover is canonical,
so we can amalgamate along such a match, where the right-hand sides
are terms of type $\applySub{T}{g \circ g^{*}f_{i}}$.

% However, the pullback also gives information to rewrite each branch $g \circ g^{*}f_{i}$ is equal in the model to
% $f_{i} \circ h$ for some $h$. So any term of type $\applySub{T}{g \circ g^{*}f_{i}}$
% also has the type $\applySub{T}{f_{i} \circ h}$, since the types have the same denotations.
% So given a term of type  $\applySub{T}{f_{i} \circ h}$ with variables from $g^{*}\D_{i}$ as the right-hand side for each branch,
% we can amalgamate them into the desired function.
% The variables in $\D_{i}$ need not all come from $\G$,
% a fact that will prove useful later when simulating the inspect idiom.
% \je{TODO explain more, example with Either/division/errors}
% \je{TODO not quite goal rewriting}




\subsection{Goal Rewriting and The Inspect Idiom}
\label{subsec:with-inspect}

The full power of with-clauses allows goal and argument types
to be rewritten: when matching intermediate $g$ against $f_{i}$, any occurrences of $g$ in the goal
or context types can be replaced by $f_{i}$.
To achieve this, we take advantage of the fact that there may be many different objects
which serve as the pullback of two arrows. Pullbacks are only are unique up to isomorphism,
and there may be many different types which are isomorphic in the model.

We can express the generalization of with-matching using one such pullback. First we note the following isomorphism:

\begin{lemma}
  If $\McC$ has extensional equality, $\Gamma \in \McC$, $T \in \Ty{\Gamma}$ and $t \in \Tm{T}$,
  then $\p^{2} : \Gamma \cext T \cext \mathsf{Id}(\applySub{T}{\p}, \v, \applySub{t}{\p}) -> \G$
  is an isomorphism.
  Moreover, $(\overline{t})^{*}(id) = \p^{2}$, i.e. the following is a pullback square:

\begin{center}
  \begin{tikzcd}
    \G\cext T \cext \mathsf{Id}(\applySub{T}{\p},\v, \applySub{t}{v}) \dar{\p^2} \rar{\p} & \Gamma \cext T \dar{id} \\
    \G \rar{\overline{t}} & \Gamma \cext T
  \end{tikzcd}
  \end{center}
\end{lemma}
That is, any context is equivalent to a context extended with a variable, once we constrain
that variable to be some term we could have made in the original context without the new variable.
Since the square is a pullback and $\{id\}$ is a canonical cover of $\Gamma \cext T$,
base change gives us that $\{p^{2}\}$ is a singleton cover of $\G$.



When we combine the above pullback with the closure of canonical coverages
under composition, we are able to case split on $t$ and  get the full version of with-matching.
Consider a canonical cover
$\{ \ext{f_{i}}{t_{i}} : \G_{i} -> \G \cext T\}$,
where each $f_{i} : \G_{i} -> \G$
and each $t_{i} \in \Tm{\applySub{T}{f_{i}}}$.
This cover is the set of patterns we want to match $t$ against.
We can apply the extension rule of \cref{subsec:cover-ext}
to introduce a fresh variable of type $\mathsf{Id}(\applySub{T}{\p}, \v, \applySub{t}{\p})$  to obtain a canonical cover:
\begin{displaymath}
  \{\ext{\ext{f_{i} \circ \p}{\applySub{t_{i}}{\p}}}{\v} :
  \G_{i} \cext \mathsf{Id}(\applySub{T}{f_{i}}, t_{i}, \applySub{t}{f_{i}})
  -> \Gamma \cext T \cext \mathsf{Id}(\applySub{T}{\p}, \v, \applySub{t}{\p})  \}
\end{displaymath}
Then, we can compose with the singleton cover $\{p^{2} : \Gamma \cext T \cext \mathsf{Id}(\applySub{T}{\p}, \v, \applySub{t}{\p}) -> \G\}$
to obtain a canonical cover:
\begin{displaymath}
  \{
  f_{i} \circ \p : \G_{i} \cext \mathsf{Id}(\applySub{T}{f_{i}}, t_{i}, \applySub{t}{f_{i}}) -> \G
  \}
\end{displaymath}
In \lang notation, the patterns
$\{ \G_{i}, (eq : t_{i} =_{\applySub{T}{f_{i}}} \applySub{t}{f_{i}}) |- f_{i} => \G \}$
can be used to define a function with arguments from $\G$,
and in each branch, we can access the variables of $\G_{i}$ and a variable
of type $t_{i} = \applySub{t}{f_{i}}$.

What does this mean for pattern matching?
First,  the different patterns $f_{i}$ came from the matching on $T$,
not on $\G$, giving the first piece we need for with-matching:
having branches that correspond to the cases for the intermediate expression,
not the function arguments.

Second, if $\McC$ has extensional equality, we can rewrite all occurrences of
$\applySub{t}{f_{i}}$ to $t_{i}$. That is, suppose we are defining
a pattern matching function with return type $S$.
Let $\G'_{i}$ be $\G_{i}$ with each occurrence of $\applySub{t}{f_{i}}$
replaced with $t_{i}$ for each $i$,
and let $S'$ be $S$ with each $t$ occurrence replaced likewise.
If for each $i$ the corresponding right hand side is
$h_{i} : \G'_{i} \cext \mathsf{Id}(\applySub{T}{f_{i}}, t_{i}, \applySub{t}{f_{i}}) -> \cdot \cext S'$,
then we also have arrows from $\G'_{i} \cext \mathsf{Id}(\applySub{T}{f_{i}}, t_{i}, \applySub{t}{f_{i}}) -> \cdot \cext S$ since having the equality proof in scope ensures
that $\G'$ and $\G$ are strictly equal in the model.
And since $\{f_{i} \circ p\}_{i}$ is a canonical cover, we can amalgamate the $h_{i}$s
into an arrow $\G -> \cdot \cext S$.

Finally, when we match on the intermediate expression, the right-hand side of
the match can access an explicit equality proof between the intermediate expression
and the right-hand side, since $\mathsf{Id}(\applySub{T}{f_{i}}, t_{i}, \applySub{t}{f_{i}})$
is in the context. Having this equality mirrors the ``inspect idiom'' commonly used alongside
with-patterns~\citep{agdacommunityWithAbstractionAgdaDocumentation2016},
and the $\mathsf{with{/}in}$ patterns added to recent version of Agda.
We can match on $t$, rewrite it to each $t_{i}$, but retain the proof that the original $t$
is equal to each $t_{i}$, so that no information is lost.
This idiom is useful if, for example, the expression $t$ arises in
a later goal and misses being rewritten the first time.

% Then we can compose with $\{p^{2} : \G \cext T \cext \mathsf{Id}(\applySub{T}{\p}, \v, \applySub{t}{\p}) -> \G \}$
% to obtain the following cover:
% \begin{displaymath}
% TODO
% \end{displaymath}

% We can apply the extension rule of \cref{TODO} to extend by a new variable of type
% $TODO$ to
% get a cover
% \begin{displaymath}
%   \{\ext{\ext{f_{i} \circ p}{\applySub{t_{i}}{\p}}}{\v} : \G_{i}  \cext \mathsf{Id}(\applySub{T}{f_{i}}, t_{i},\applySub{t}{\p \circ f_{i}} ) -> \Gamma \cext T \cext \mathsf{Id}(\applySub{T}{\p}, \v, \applySub{t}{\p})\}
%   \end{displaymath}
%   Finally, we can apply the composition rule and the CwF laws to get a cover \je{TODO}
% \begin{displaymath}
%   \{ f_{i} \circ \p : \G_{i}  \cext \mathsf{Id}(\applySub{T}{f_{i}}, t_{i},\applySub{t}{\p \circ f_{i}} ) -> \Gamma \}
%   \end{displaymath}


% In terms of pattern matching, this means two things. First,
% when $\Gamma$ is a scrutinee type, for any intermediate term $t$ we can generalize
% occurences of $t$ to a fresh variable.
% This is because the context of $\p^{2}$ has a varible of type $T$, which,
% if $\McC$ is extensional, must be exactly equal in the model to $\applySub{t}{\v}$.
% So replacing $t$ with the fresh variable $\v$ in both the argument types and the goal
% type is a no-op, since they are the exact same objects in the model.

% Second, the right hand side can make explicit references to a proof
% that the new variable $\v$ is equal to $t$


Something strange has happened: we have conjured a new variable
of an equality type out of thin air.
It does not correspond to
any part of the arguments of the function we are defining, but nevertheless, since
the arrow is a canonical cover, we can refer to it on the right-hand side
of the pattern match and still amalgamate to a well-defined term.
In essence, base change says that in addition to matching on the input, we can
match on things we build from that input and include them in our context as
if they were part of the input, giving exactly what we need for with-matching.


The above construction only works for with-expressions matching on single terms, since
the equality type operates on terms, not arrows. However, if $\McC$ is democratic
(i.e. every context is equivalent to some closed type), then we can convert arrows
to terms and have with-matching on multiple values at once.

% \subsubsection{Uniqueness of Identity Proofs}
% \label{subsec:uip}


==> main-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}A matching family for $\singleton {\iota }$ is just an element of $x \in P(\Gamma )$. We can use $P(\iota ^{-1})(x)$ as our amalgamation, and since $P$ is a functor, $P(\iota )(P(\iota ^{-1})(x)) = P(\iota ^{-1}\circ \iota )(x) = P(id)(x) = x$. Every presheaf is thus a sheaf for $\singleton {\iota }$, so every representable is, so the largest coverage with all representables as sheaves must contain all isomorphisms.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}Recall that for $\setj {j \in I}{ \inj _{j} : \Delta _{j} -> \coprod _{i \in I}\Delta _{i} }$ to be in the canonical coverage, for every $\Gamma $ and every $g : \Xi -> \coprod _{i \in I}\Delta _{i}$, $\yo (\Gamma )$ should be a sheaf for $\setj {j \in I}{ g*\inj _{j} }$. So for each $j$ there is pullback diagram that looks like this: \par \begin {center} \begin {tikzcd} g^{*} ( \Delta _j) \rar {} \dar {g^{*} (\inj _j)} & \Delta _j \dar {\inj _j} \\ \Xi \rar {g} & \coprod _{i \in I} \Delta _i \end {tikzcd} \end {center} \par Since the identity always has a pullback and $\coprod _{i \in I} \inj _i = id$, we have the following pullback diagram: \begin {center} \begin {tikzcd} \Xi \rar {g} \dar {id} & \coprod _{i \in I}\Delta _i \dar {\coprod _{i \in I} \inj _i} \\ \Xi \rar {g} & \coprod _{i \in I} \Delta _i \end {tikzcd} \end {center} \par Since $\McC $ preserves coproducts under pullback, this means that there is an isomorphism $\iota : \Xi \cong \coprod _{i \in I} (g^{*}\inj _{i})$, and we have the following pullback diagram: \par \begin {center} \begin {tikzcd} \coprod _{i \in I} (g^{*} \Delta _i) \rar { g \circ \coprod _{i \in I}(g^{*}\inj _i)} \dar { \coprod _{i \in I} (g^{*} \inj _i)} & \coprod _{i \in I}\Delta _i \dar {\coprod _{i \in I} \inj _i} \\ \Xi \arrow [u, bend left, "\iota "] \rar {g} & \coprod _{i \in I} \Delta _i \end {tikzcd} \end {center} \par \par Let's return to the sheaf condition. Consider some $\setj {j \in I}{x_{j} : g^{*}\Delta _{j} -> \Gamma }$. For $\yo (\Gamma )$ to be a sheaf for $\setj { g^{*} \inj _{j}}$, there should be a unique $x : \Xi -> \Gamma $ such that $x \circ g^{*}\inj _{j} = x_{j}$. The universal property of the coproduct gives us a unique $\coprod _{i \in I}(x_{i}) : \coprod _{i \in I}(g^{*}\Delta _{i}) -> \Gamma $. We can then set $x := \coprod _{i \in I}(x_{i}) \circ \iota $. \par First we must prove that $x$ respect each $\inj _{j}$. We have $x \circ g^{*}\inj _{j} = \coprod _{i \in I}(x_{i}) \circ \iota \circ g^{*}\inj _{j}$, so it suffices to show that $\iota \circ g^{*}\inj _{j} = \inj _{j} : g^{*}\Delta _{j} -> \coprod _{i \in I} g^{*}\Delta _{i}$. We have $id_{\coprod _{i \in I} g^{*}\Delta _{i}} = \iota \circ \coprod _{i \in I}(g^{*}\inj _{i}) = \coprod _{i \in I}(\iota \circ g^{*}\inj _{i})$, so $\inj _{j} = id_{\coprod _{i \in I} g^{*}\Delta _{i}} \circ \inj _{j} = \coprod _{i \in I}(\iota \circ g^{*}\inj _{i}) \circ \inj _{j} = \iota \circ g^{*}\inj _{j}$. \par All that remains is to show the uniqueness of $x$. Suppose we have $y : \Xi -> \Gamma $ such that $y \circ g^{*}\inj _{j} = x_{j}$. Then $y = y \circ \coprod _{i \in I}(g^{*}\inj _{i}) \circ \iota = \coprod _{i \in I} (y \circ g^{*}\inj _{i}) \circ \iota = \coprod _{i \in I}(x_{i}) \circ \iota = x$.\end{proof}

\prAtEndRestateiv*

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}The arrow $\iota $ is necessarily an isomorphism by the uniqueness of initial objects, so we can use \cref {thm:cover-comp} replace $\theta $ with $0_{\Gamma }$ and still have a canonical cover. We need to show that for any $g : \Xi -> \Gamma $ and any motive $M \in \McC $, $\yo (M)$ is a sheaf for $g^{*}(c \setminus \singleton {\theta })$. We have $g^{*}(0_{\Gamma }) = 0_{\Xi }$ by the uniqueness of initial arrows So in a matching family for $\yo (M)$, the only possible value in $\yo (M)(g^{*}(0_{\Gamma })) $ is $0_{M}$. So given a matching family for $g^{*}(c \setminus \singleton {\theta })$, we can always construct one for $g^{*}(c)$, which we know is a canonical cover, and hence we can amalgamate for.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\D := \ext {\ext {\overline {t_{1}\sub {p}}}{t_{2}\sub {p}}}{\v }^{*} \Gamma \cext T$. Both arrows out of $\D $ in the pullback square are into extended contexts, so they are necessarily equal to extended morphisms. So our pullback square looks like this for some $\theta , \sigma : \D -> \G $, $t_{Id} \in \Tm {\mathsf {Id}(T,t_{1},t_{2})\sub {\theta }}$ and $t_{12} \in \Tm {\applySub {T}{\sigma }}$: \begin {center} \begin {tikzcd} \Delta \rar {\ext {\sigma }{t_{12}}} \dar {\ext {\theta }{t_{Id}}} & \Gamma \cext T \dar {\mathsf {Refl}_T}\\ \Gamma \cext \mathsf {Id}(T,t_1,t_2) \rar {\ext {\ext {\overline {t_1}}{t_2}}{\v }} & \G \cext T \cext \applySub {T}{\p } \cext \mathsf {Id}(T) \end {tikzcd}\\ \end {center} Applying our CwF laws we get $\ext {\ext {\ext {\theta }{\applySub {t_{1}}{\theta }}}{\applySub {t_{2}}{\theta }}}{t_{Id}} = \mathsf {Refl}_{T}\circ \ext {\sigma }{t_{12}} $. Then precomposing with $\p $ on both sides yields $\ext {\ext {\theta }{\applySub {t_{1}}{\theta }}}{\applySub {t_{2}}{\theta }} = \ext {\ext {\sigma }{t_{12}}}{t_{12}}$, so we have $\theta = \sigma $ and $\applySub {t_{1}}{\theta } = t_{12} = \applySub {t_{2}}{\theta }$. Likewise, applying both sides as substitutions to $\v $ gives $t_{Id} = \applySub {\v }{\mathsf {Refl}_{T}\circ \ext {\sigma }{t_{12}} } = \mathsf {Refl}_{T\sub {\theta }}(t_{12}) $ by the previous equations and the stability of $\mathsf {Refl}$ under substitution. \je {TODO stability of Refl under subst} \par Finally, we have $\singleton {\ext {\theta }{\mathsf {Refl}_{T}(t_{12})}}$ as a canonical cover by the base change theorem. \par \end{proof}


==> oldmacros.tex <==
% Joey's generic macros
% shared across documents
\usepackage{amsmath}
\usepackage{xparse}

\usepackage{mathpartir}
\usepackage[capitalise]{cleveref}

%% Some recommended packages.
\usepackage{booktabs}   %% For formal tables:
                        %% http://ctan.org/pkg/booktabs
% \usepackage{subcaption} %% For complex figures with subfigures/subcaptions
                        %% http://ctan.org/pkg/subcaption
\usepackage{csquotes}
\usepackage{fancyvrb}
\usepackage{stmaryrd}
\usepackage{adjustbox}
\usepackage{xspace}
\usepackage{relsize}
% \usepackage{listings}
\usepackage{comment}

\usepackage{savesym}
\savesymbol{program}
\usepackage{amsmath}
\usepackage{semantic}
\usepackage{mdframed}
% \usepackage[dvipsnames]{xcolor}
% \usepackage{proof-at-the-end}
% \usepackage{hyperref}
% \usepackage[capitalise]{cleveref}

% \newtheorem{desiderata}{Desiderata}
% \numberwithin{desiderata}{section}
% \crefname{desiderata}{Desideratum}{Desiderata}

\usepackage[geometry]{ifsym}

%%% Proofs in the appendix

% \usepackage{bm}


% Custom mathBB

\newcommand\doubleplus{+\kern-1.3ex+\kern0.8ex}
\newcommand\mdoubleplus{\ensuremath{\mathbin{+\mkern-5mu+}}}

\newcommand\codeFont[1]{\mathtt{#1}}

\NewDocumentCommand\defineMeta{mmmm}{%
    \expandafter\DeclareDocumentCommand\csname#1#2\endcsname{ E{^_}{{}{}} }{%
    #3{#4^{#3{##1}}_{#3{##2}}}%
    }%
}
\NewDocumentCommand\sgMeta{mG{#1}}{
    \defineMeta{g}{#1}{\gradualstyle}{#2}
    \defineMeta{s}{#1}{\staticstyle}{#2}
    \defineMeta{r}{#1}{\surfstyle}{#2}
}


\NewDocumentCommand\defineStaticFun{mG{#1}}{%
    \expandafter\NewDocumentCommand\csname#1\endcsname{od()}{%
    \staticstyle{\mathtt{#2}\ {\IfNoValueF{##1}{##1}}{\IfNoValueF{##2}{(##2)}} }
    }%
}


%\sgMeta{x} Gives us \gx and \sx commands
%properly styled for the gradual and static languages
%Optional second argument is how to display the varible, defaults to first argument
\sgMeta{x}
\sgMeta{y}
\sgMeta{z}
\sgMeta{C}
\sgMeta{D}
\sgMeta{N}
\sgMeta{M}
\sgMeta{ff}{f}
\sgMeta{pf}{p}
\sgMeta{P}
\sgMeta{el}{\overline{e}}
\sgMeta{X}
\sgMeta{Y}
\sgMeta{Z}
\sgMeta{t}
\sgMeta{T}
\sgMeta{s}
\sgMeta{S}
\sgMeta{m}
\sgMeta{n}
\sgMeta{u}
\sgMeta{U}
\sgMeta{v}
\sgMeta{V}
\sgMeta{A}
\sgMeta{B}
\sgMeta{J}{\text{J}}
\sgMeta{Nat}{\text{Nat}}
\sgMeta{Int}{\text{Int}}
\sgMeta{Bool}{\text{Bool}}
\sgMeta{Zero}{0}
\sgMeta{NatElim}{\text{NatElim}}
\sgMeta{VecElim}{\text{EqElim}}
\sgMeta{EqElim}{\text{VecElim}}
\sgMeta{Refl}{\text{Refl}}
\sgMeta{subst}{\text{subst}}

\sgMeta{G}{\Gamma}
\sgMeta{ep}{\varepsilon}
\sgMeta{times}{\times}
\sgMeta{lambda}{\lambda}
\sgMeta{Unit}{\mathbf{1}}
\sgMeta{unit}{()}

\sgMeta{spine}{\seq{e}}

\mathlig{||}{\bnfalt}
\mathlig{::=}{\bnfdef}
\mathlig{+::=}{\bnfadd}
\mathlig{-::=}{\bnfsub}
\mathlig{|>}{\vartriangleright}
\mathlig{<|}{\vartriangleleft}
\mathlig{<=}{\Leftarrow}
\mathlig{=>}{\Rightarrow}
% \mathlig{~>}{\leadsto}
\mathlig{>->}{\rightarrowtail}
\mathlig{|->}{\mapsto}
% \mathlig{++}{\mdoubleplus}
\mathlig{|=>}{\Mapsto}
\mathlig{==}{=}
% \mathlig{=-=}{\cong}
\mathlig{**}{\times}
\mathlig{<<}{\langle}
\mathlig{>>}{\rangle}

\mathlig{|=}{\vDash}
\newcommand{\set}[1]{{\{ #1 \}}}
\newcommand{\ep}{\varepsilon}

\newcommand{\gmu}{\gradualstyle{\tilde{\mu}}}


% \NewDocumentCommand{\stt}{m}{\staticstyle{\ensuremath{\mathtt{#1}}}}
% \NewDocumentCommand{\gtt}{m}{\gradualstyle{\ensuremath{\mathtt{#1}}}}

\newcommand{\sto}{\staticstyle{\to}}
\newcommand{\gto}{\gradualstyle{\to}}

% \newcommand\gcode[1]{\gradualstyle{\texttt{#1}}}
% \newcommand\scode[1]{\staticstyle{\texttt{#1}}}
\renewcommand{\P}{\mathcal{P}}

\newcommand{\mynote}[3][red]
    {{\color{#1} \fbox{\bfseries\sffamily\scriptsize#2}
    {\small$\blacktriangleright$\textsf{\emph{#3}}$\blacktriangleleft$}}~}
% \newcommand{\et}[1]{\mynote{ET}{#1}}
\newcommand{\je}[1]{\mynote{JE}{#1}}
% \newcommand{\et}[1]{}
% \newcommand{\je}[1]{}
\newcommand{\ron}[1]{\mynote{RG}{#1}}

% \usepackage{inconsolata}
\usepackage{mathtools}

\usepackage{pifont}
\newcommand{\cmark}{{\color{Emerald}\ding{51}}}%
\newcommand{\xmark}{{\color{RedOrange}\ding{55}}}%


\newcommand{\gradualcolor}{\color{RoyalBlue}}
\newcommand{\surfcolor}{\color{Emerald}}
\newcommand{\staticcolor}{\color{RedOrange}}

\newcommand{\gradualstyle}[1]{{\ensuremath{\gradualcolor\mathbf{{#1}}}}}
\newcommand{\surfstyle}[1]{{\ensuremath{\surfcolor\mathit{{#1}}}}}
\newcommand{\staticstyle}[1]{{\ensuremath{\staticcolor\mathsf{{#1}}}}}

\newcommand{\staticdesc}{\staticstyle{\textsf{red sans-serif font}}\xspace}
\newcommand{\gradualdesc}{\gradualstyle{\textbf{blue, bold serif font}}\xspace}
% \newcommand{\surfdesc}{\surfstyle{\textit{green, italic serif font}}\xspace}

\newcommand{\g}[1]{\gradualstyle{#1}}
\newcommand{\s}[1]{\staticstyle{#1}}
\renewcommand{\r}[1]{\surfstyle{#1}}
\newcommand{\ix}[1]{\color{black}{\mathit{#1}}}

\NewDocumentCommand{\sType}{m}{{\staticstyle{\textbf{\textsf{Type}}_{#1}}}}
\NewDocumentCommand{\gType}{m}{{\gradualstyle{\mathbf{Type}_{#1}}}}
\NewDocumentCommand{\rType}{m}{{\surfstyle{\textbf{\textit{Type}}_{#1}}}}


\newcommand{\typeType}[1]{\mathcal{U}_{#1}}

\newcommand{\stepstostar}{\longrightarrow^{*}}
\newcommand{\stepstoplus}{\longrightarrow^{+}}
\newcommand{\etasteps}{\longrightarrow^{*}_{\eta}}
\newcommand{\stepsto}{\longrightarrow}


\newcommand{\guarded}{\s{\triangleright}}
\newcommand{\tguarded}{\s{\blacktriangleright}}
\newcommand{\gapp}{\s{\circledast}}
\newcommand{\aeguarded}{\s{\triangleright_{\ae}}}
\newcommand{\aetguarded}{\s{\blacktriangleright_{\ae}}}
\newcommand{\aegapp}{\s{\circledast_{\ae}}}
\newcommand{\LAE}{\s{\mathcal{L}_\ae}}

%https://github.com/wilbowma/dissertation/blob/0454bdb171c95d826561703231930c23b8241d6e/defs.tex
\newenvironment{bnfgrammar}
{\begin{displaymath}\begin{array}{lrcl}}
{\end{array}\end{displaymath}}
\newcommand{\bnfnewline}{
  \\[6pt]
}
\newcommand{\bnflabel}[1]{\mbox{\textit{#1}}}
\newcommand{\bnfalt}{\mathbf{\,\,\mid\,\,}}
\newcommand{\bnfdef}{\mathbf{\ \Coloneqq\ }}
\newcommand{\defbnf}{\bnfdef} % fd is my vim-escape combo
\newcommand{\bnfadd}{{\mathbf{\ +\!\!\Coloneqq\ }}}
\newcommand{\bnfsub}{{\bf - : : =}}

\makeatletter
\newcommand{\mathboxed}[1]{\text{\fboxsep=.2em\fbox{\m@th$\displaystyle#1$}}}
\makeatother

\newcommand{\ie}{i.e.\xspace}
\newcommand{\eg}{e.g.\xspace}

\newcommand{\errsym}{\mho}
\newcommand\gqm{\gradualstyle{\normalfont{\textbf{?}}}}
\newcommand\rqm{\surfstyle{\normalfont{\textbf{?}}}}
\newcommand\rqmat[1]{\surfstyle{\normalfont{\textit{?}}_{@#1}}}
\newcommand\gqmat[1]{\gradualstyle{\normalfont{\textbf{?}}_{#1}}}
% \newcommand\qm{\mathbb{?} }
\newcommand\err{\gradualstyle{\errsym}}
\newcommand\errat[1]{\gradualstyle{\errsym}_{\g{#1}}}
\newcommand\errl{\gradualstyle{\errsym_{\ell}}}
\newcommand{\bbb}{\mathbb{B}}
\newcommand{\If}{\mathbf{if}}
\newcommand{\true}{\mathbf{true}}
\newcommand{\false}{\mathbf{false}}
\newcommand{\Type}{\mathbf{Type}}



\newcommand{\K}{$\mathbf{K}$ }
\newcommand{\UIP}{$\mathbf{UIP}$ }

\newcommand{\abe}{{\alpha\beta\eta}}

\newcommand{\rrule}{\textsc}


\newcommand\blackoline[1]{\colorlet{temp}{.}\color{black}\overrightarrow{\color{temp}#1}\color{temp}}
\newcommand{\seq}[1]{\overrightarrow{#1}}

\newcommand{\ala}{\`a la }

\NewDocumentCommand{\tr}{}{\staticstyle{tr}}
\newcommand{\trUp}{\ensuremath{\tr^{\s\uparrow}}}
\newcommand{\trDown}{\ensuremath{\tr^{\s\downarrow}}}

% \newcommand{\sqube}{\sqsubseteq}
% \newcommand{\sqeq}{\sqsupseteq\sqsubseteq}
\newcommand{\bZero}{{\mathbb{0}}}
\newcommand{\bOne}{{\mathbb{1}}}
\newcommand{\bN}{{\mathbb{N}}}
\newcommand{\bC}{{\mathbb{C}}}
\newcommand{\bB}{{\mathbb{B}}}


% Stolen from Felipe's \AGT paper
\definecolor{lightgray}{gray}{0.90}
\newcommand{\Gbox}[1]{\colorbox{lightgray}{$#1$}}

\newcommand{\gbox}[1]{%
  {\setlength{\fboxsep}{1pt}\colorbox{lightgray}{\tiny$#1$}}}

\usepackage{ulem}
\newcommand{\change}[1]{#1}
% \newcommand{\change}[1]{{\color{orange}\uline{#1}}}

\newcommand{\Godel}{G\"{o}del}


\newmdenv[
usetwoside=false,
topline=false,
bottomline=false,
rightline=false,
leftmargin=0.2in,
linewidth=0.75pt,
skipabove=\topsep,
skipbelow=\topsep,
nobreak=false
]{leftrule}


% stolen from https://arxiv.org/abs/1911.00583
\newcommand{\case}[2]{
  \noindent $\blacktriangleright$ \textbf{Case} \text{#1} \textbf{:}
  {
    % \setlength{\parskip}{0.7em}
    \begin{leftrule}
      % \vspace{0.35em}
      #2
    \end{leftrule}
  }
  \noindent \ignorespaces
}

\newcommand{\lcase}[2]{
  \noindent $\blacktriangleright$ \textbf{Case} \text{#1} \textbf{:} #2
}

\newcommand{\mcase}[2]{\case{$#1$}{#2}}


\newcommand{\rlcase}[2]{\lcase{\rrule{#1}}{#2}}
\newcommand{\mlcase}[2]{\lcase{$#1$}{#2}}

\newcommand{\rcase}[2]{\case{\rrule{#1}}{#2}}



\newsavebox{\saveboxedarray}
\newenvironment{inferbox}[0]
{\begin{minipage}{\textwidth}\mprset{center}\begin{mathpar}}
    {\end{mathpar}\end{minipage}}
\newenvironment{syntaxcategory}[1]
{\begin{array}{lcll} \multicolumn{4}{l}{\mbox{\textbf{#1}}}\\}
   {\end{array}}
 \newenvironment{boxedarray}[1]
 {\begin{lrbox}{\saveboxedarray}\begin{math}\begin{array}{#1}}
                                              {\end{array}\end{math}\end{lrbox}{\usebox{\saveboxedarray}}}
                                        \reservestyle{\command}{\textsf}

% \newsavebox{\saveboxedarray}
% \newenvironment{inferbox}[0]
% {\begin{minipage}{\textwidth}\mprset{center}\begin{mathpar}}
%     {\end{mathpar}\end{minipage}}
% \newenvironment{syntaxcategory}[1]
% {\begin{array}{lcll} \multicolumn{4}{l}{\mbox{\textbf{#1}}}\\}
%    {\end{array}}
%  \newenvironment{boxedarray}[1]{}{}
%                                         \reservestyle{\command}{\textsf}

\newcommand{\myparagrapht}[1]{\noindent{\bf #1}}
\newcommand{\myparagraph}[1]{\vspace{0.5em}\myparagrapht{#1.}}


% \newcommand*\circled[1]{\tikz[baseline=(char.base)]{
%   \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}

\usepackage{wrapfig}

\newcommand{\cst}{\cong}

% \newcommand{\qm}{ { \textbf{?}TODO }}

%TODO: define this to link back?
\newcommand{\defn}[1]{\textit{\gls{#1}}}

